Is Spectral Width a Reliable Measure of GRB Emission Physics?

The spectral width and sharpness of unfolded, observed GRB spectra have been presented as a new tool to infer physical properties about GRB emission via spectral fitting of empirical models. Following the tradition of the 'line-of-death', the spectral width has been used to rule out synchrotron emission in a majority of GRBs. This claim is investigated via reexamination of previously reported width measures. Then, a sample of peak-flux GRB spectra are fit with an idealized, physical synchrotron model. It is found that many spectra can be adequately fit by this model even when the width measures would reject it. Thus, the results advocate for fitting a physical model to be the sole tool for testing that model. Finally, a smoothly-broken power law is fit to these spectra allowing for the spectral curvature to vary during the fitting process in order to understand why the previous width measures poorly predict the spectra. It is found that the failing of previous width measures is due to a combination of inferring physical parameters from unfolded spectra as well as the presence of multiple widths in the data beyond what the Band function can model.

==> table_res.tex <==
\begin{tabular}{lllllllll}
\toprule
{} &               band\_alpha &               sbpl\_alpha &              sbpl\_delta & DIC\_delta & pDIC\_band & pDIC\_sbpl &    band\_ppc &    sync\_ppc \\
\midrule
GRB080817161 &  \$-0.78\_\{-0.08\}\textasciicircum\{+0.08\}\$ &  \$-0.79\_\{-0.22\}\textasciicircum\{+0.26\}\$ &  \$0.53\_\{-0.53\}\textasciicircum\{+0.35\}\$ &      9.01 &      5.79 &     -1.51 &       0.184 &       0.144 \\
GRB080906212 &  \$-0.33\_\{-0.07\}\textasciicircum\{+0.07\}\$ &  \$-0.60\_\{-0.13\}\textasciicircum\{+0.10\}\$ &  \$0.35\_\{-0.14\}\textasciicircum\{+0.14\}\$ &      6.10 &      6.52 &      5.43 &       0.196 &       0.004 \\
GRB080925775 &  \$-0.63\_\{-0.10\}\textasciicircum\{+0.08\}\$ &  \$-0.77\_\{-0.23\}\textasciicircum\{+0.15\}\$ &  \$0.44\_\{-0.27\}\textasciicircum\{+0.21\}\$ &      5.27 &      5.62 &      2.92 &       0.172 &       0.150 \\
GRB081215784 &  \$-0.58\_\{-0.02\}\textasciicircum\{+0.02\}\$ &  \$-0.46\_\{-0.09\}\textasciicircum\{+0.06\}\$ &  \$0.83\_\{-0.16\}\textasciicircum\{+0.12\}\$ &     19.71 &      6.91 &      5.14 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB090131090 &  \$-0.55\_\{-0.16\}\textasciicircum\{+0.12\}\$ &   \$0.37\_\{-1.26\}\textasciicircum\{+0.78\}\$ &  \$0.76\_\{-0.44\}\textasciicircum\{+0.23\}\$ &      1.88 &     -6.96 &     -5.12 &       0.046 &       0.026 \\
GRB090620400 &   \$0.14\_\{-0.10\}\textasciicircum\{+0.10\}\$ &  \$-0.03\_\{-0.30\}\textasciicircum\{+0.20\}\$ &  \$0.51\_\{-0.24\}\textasciicircum\{+0.15\}\$ &      9.40 &      5.99 &      1.55 &       0.042 &  \$<10\textasciicircum\{-3\}\$ \\
GRB090626189 &  \$-0.35\_\{-0.10\}\textasciicircum\{+0.09\}\$ &   \$0.15\_\{-0.86\}\textasciicircum\{+0.48\}\$ &  \$0.90\_\{-0.52\}\textasciicircum\{+0.37\}\$ &     24.69 &      4.53 &    -20.26 &       0.712 &       0.310 \\
GRB090809978 &  \$-0.50\_\{-0.08\}\textasciicircum\{+0.08\}\$ &  \$-0.74\_\{-0.15\}\textasciicircum\{+0.10\}\$ &  \$0.28\_\{-0.28\}\textasciicircum\{+0.12\}\$ &      6.62 &      5.98 &      3.38 &       0.658 &       0.384 \\
GRB090820027 &  \$-0.53\_\{-0.03\}\textasciicircum\{+0.03\}\$ &  \$-0.66\_\{-0.06\}\textasciicircum\{+0.06\}\$ &  \$0.45\_\{-0.12\}\textasciicircum\{+0.07\}\$ &     25.51 &      5.91 &     -2.66 &       0.004 &  \$<10\textasciicircum\{-3\}\$ \\
GRB090829672 &  \$-1.13\_\{-0.04\}\textasciicircum\{+0.04\}\$ &  \$-1.26\_\{-0.04\}\textasciicircum\{+0.03\}\$ &  \$0.21\_\{-0.12\}\textasciicircum\{+0.13\}\$ &      9.58 &      5.90 &      5.90 &       0.004 &  \$<10\textasciicircum\{-3\}\$ \\
GRB091003191 &  \$-0.56\_\{-0.06\}\textasciicircum\{+0.06\}\$ &  \$-0.49\_\{-0.24\}\textasciicircum\{+0.14\}\$ &  \$0.79\_\{-0.41\}\textasciicircum\{+0.22\}\$ &     24.86 &      5.45 &    -14.41 &       0.412 &       0.318 \\
GRB091127976 &  \$-1.13\_\{-0.05\}\textasciicircum\{+0.05\}\$ &  \$-0.70\_\{-0.35\}\textasciicircum\{+0.27\}\$ &  \$1.28\_\{-0.37\}\textasciicircum\{+0.28\}\$ &     24.09 &      5.95 &    -18.80 &       0.260 &       0.226 \\
GRB100131730 &  \$-0.28\_\{-0.10\}\textasciicircum\{+0.09\}\$ &  \$-0.53\_\{-0.21\}\textasciicircum\{+0.15\}\$ &  \$0.35\_\{-0.23\}\textasciicircum\{+0.18\}\$ &      6.67 &      5.76 &      4.03 &       0.790 &       0.426 \\
GRB100701490 &  \$-0.61\_\{-0.04\}\textasciicircum\{+0.04\}\$ &  \$-0.58\_\{-0.11\}\textasciicircum\{+0.08\}\$ &  \$0.71\_\{-0.27\}\textasciicircum\{+0.22\}\$ &      8.83 &      5.83 &     -2.53 &       0.338 &       0.156 \\
GRB100719989 &  \$-0.57\_\{-0.04\}\textasciicircum\{+0.04\}\$ &  \$-0.21\_\{-0.23\}\textasciicircum\{+0.19\}\$ &  \$1.10\_\{-0.32\}\textasciicircum\{+0.27\}\$ &     33.40 &      5.90 &    -11.16 &       0.004 &  \$<10\textasciicircum\{-3\}\$ \\
GRB101014175 &  \$-0.90\_\{-0.04\}\textasciicircum\{+0.04\}\$ &   \$0.16\_\{-0.71\}\textasciicircum\{+0.40\}\$ &  \$2.63\_\{-1.05\}\textasciicircum\{+0.76\}\$ &     83.79 &      5.27 &    -46.02 &       0.096 &       0.092 \\
GRB110301214 &  \$-0.95\_\{-0.03\}\textasciicircum\{+0.03\}\$ &  \$-1.11\_\{-0.07\}\textasciicircum\{+0.05\}\$ &  \$0.43\_\{-0.09\}\textasciicircum\{+0.11\}\$ &     11.69 &      6.80 &      1.73 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB110625881 &  \$-0.53\_\{-0.03\}\textasciicircum\{+0.04\}\$ &  \$-0.36\_\{-0.27\}\textasciicircum\{+0.19\}\$ &  \$0.80\_\{-0.30\}\textasciicircum\{+0.23\}\$ &     25.06 &      6.97 &     -9.94 &       0.128 &       0.006 \\
GRB110921912 &  \$-0.64\_\{-0.06\}\textasciicircum\{+0.05\}\$ &   \$0.49\_\{-0.74\}\textasciicircum\{+0.46\}\$ &  \$2.10\_\{-0.63\}\textasciicircum\{+0.65\}\$ &     34.57 &      5.32 &    -14.51 &       0.066 &       0.084 \\
GRB120102095 &  \$-1.06\_\{-0.09\}\textasciicircum\{+0.08\}\$ &  \$-1.08\_\{-0.19\}\textasciicircum\{+0.21\}\$ &  \$0.60\_\{-0.60\}\textasciicircum\{+0.45\}\$ &      9.97 &      3.38 &     -4.15 &       0.902 &       0.900 \\
GRB120217904 &  \$-0.78\_\{-0.07\}\textasciicircum\{+0.06\}\$ &  \$-0.91\_\{-0.11\}\textasciicircum\{+0.07\}\$ &  \$0.37\_\{-0.20\}\textasciicircum\{+0.18\}\$ &      8.73 &      6.45 &      3.91 &       0.566 &       0.606 \\
GRB120707800 &  \$-0.90\_\{-0.11\}\textasciicircum\{+0.10\}\$ &  \$-0.59\_\{-0.66\}\textasciicircum\{+0.44\}\$ &  \$0.84\_\{-0.70\}\textasciicircum\{+0.45\}\$ &     14.31 &      4.86 &     -9.81 &       0.176 &       0.158 \\
GRB120711115 &  \$-0.86\_\{-0.04\}\textasciicircum\{+0.04\}\$ &  \$-0.88\_\{-0.12\}\textasciicircum\{+0.08\}\$ &  \$0.59\_\{-0.42\}\textasciicircum\{+0.37\}\$ &     18.55 &      5.76 &    -14.57 &       0.562 &       0.422 \\
GRB120921877 &   \$0.73\_\{-0.29\}\textasciicircum\{+0.24\}\$ &   \$1.21\_\{-0.31\}\textasciicircum\{+0.79\}\$ &  \$0.69\_\{-0.22\}\textasciicircum\{+0.23\}\$ &     -5.04 &     -3.63 &      4.71 &       0.042 &  \$<10\textasciicircum\{-3\}\$ \\
GRB130606497 &  \$-1.06\_\{-0.02\}\textasciicircum\{+0.01\}\$ &  \$-0.95\_\{-0.06\}\textasciicircum\{+0.05\}\$ &  \$1.20\_\{-0.23\}\textasciicircum\{+0.21\}\$ &     20.49 &      5.92 &     -1.13 &       0.040 &  \$<10\textasciicircum\{-3\}\$ \\
GRB130704560 &  \$-0.90\_\{-0.04\}\textasciicircum\{+0.05\}\$ &  \$-0.90\_\{-0.15\}\textasciicircum\{+0.13\}\$ &  \$0.63\_\{-0.14\}\textasciicircum\{+0.11\}\$ &      3.14 &      4.60 &      5.47 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB130815660 &  \$-0.63\_\{-0.07\}\textasciicircum\{+0.07\}\$ &  \$-0.92\_\{-0.10\}\textasciicircum\{+0.07\}\$ &  \$0.25\_\{-0.11\}\textasciicircum\{+0.09\}\$ &      7.52 &      6.41 &      5.34 &       0.002 &       0.002 \\
GRB131028076 &  \$-0.33\_\{-0.24\}\textasciicircum\{+0.78\}\$ &  \$-0.60\_\{-0.03\}\textasciicircum\{+0.03\}\$ &  \$0.55\_\{-0.06\}\textasciicircum\{+0.06\}\$ &   1955.85 &   -169.51 &      6.02 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB131127592 &  \$-0.77\_\{-0.04\}\textasciicircum\{+0.05\}\$ &  \$-0.99\_\{-0.10\}\textasciicircum\{+0.08\}\$ &  \$0.38\_\{-0.15\}\textasciicircum\{+0.12\}\$ &     16.32 &      6.60 &     -4.45 &       0.024 &       0.022 \\
GRB140206304 &   \$0.49\_\{-0.24\}\textasciicircum\{+0.19\}\$ &   \$1.24\_\{-0.32\}\textasciicircum\{+0.74\}\$ &  \$0.73\_\{-0.16\}\textasciicircum\{+0.20\}\$ &      2.58 &     -3.03 &      2.96 &       0.506 &       0.002 \\
GRB140209313 &  \$-0.00\_\{-0.14\}\textasciicircum\{+0.14\}\$ &   \$0.23\_\{-0.77\}\textasciicircum\{+0.49\}\$ &  \$0.77\_\{-0.51\}\textasciicircum\{+0.30\}\$ &     11.28 &      3.47 &     -4.71 &       0.162 &       0.026 \\
GRB150105257 &  \$-0.87\_\{-0.13\}\textasciicircum\{+0.11\}\$ &  \$-0.90\_\{-0.43\}\textasciicircum\{+0.54\}\$ &  \$0.44\_\{-0.44\}\textasciicircum\{+0.34\}\$ &      5.47 &      2.67 &     -1.37 &       0.314 &       0.288 \\
GRB150201574 &  \$-0.67\_\{-0.03\}\textasciicircum\{+0.04\}\$ &  \$-0.97\_\{-0.05\}\textasciicircum\{+0.05\}\$ &  \$0.26\_\{-0.06\}\textasciicircum\{+0.06\}\$ &     12.53 &      5.93 &      6.92 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB150213001 &  \$-1.22\_\{-0.02\}\textasciicircum\{+0.02\}\$ &  \$-1.51\_\{-0.02\}\textasciicircum\{+0.02\}\$ &  \$0.20\_\{-0.04\}\textasciicircum\{+0.04\}\$ &     52.70 &      7.03 &      6.62 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB150314205 &  \$-0.33\_\{-0.04\}\textasciicircum\{+0.04\}\$ &  \$-0.36\_\{-0.13\}\textasciicircum\{+0.10\}\$ &  \$0.56\_\{-0.15\}\textasciicircum\{+0.11\}\$ &     15.87 &      5.81 &      1.90 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB150330828 &  \$-0.88\_\{-0.03\}\textasciicircum\{+0.03\}\$ &  \$-1.02\_\{-0.04\}\textasciicircum\{+0.03\}\$ &  \$0.27\_\{-0.11\}\textasciicircum\{+0.12\}\$ &     13.57 &      6.76 &      4.64 &       0.002 &  \$<10\textasciicircum\{-3\}\$ \\
GRB150627183 &  \$-0.79\_\{-0.03\}\textasciicircum\{+0.04\}\$ &  \$-0.99\_\{-0.05\}\textasciicircum\{+0.04\}\$ &  \$0.27\_\{-0.10\}\textasciicircum\{+0.08\}\$ &     12.08 &      5.84 &      5.40 &       0.136 &       0.104 \\
GRB150824079 &  \$-0.42\_\{-0.06\}\textasciicircum\{+0.07\}\$ &  \$-0.11\_\{-0.35\}\textasciicircum\{+0.28\}\$ &  \$1.10\_\{-0.40\}\textasciicircum\{+0.35\}\$ &     24.03 &      6.44 &     -8.87 &       0.290 &       0.108 \\
GRB160101030 &  \$-0.80\_\{-0.04\}\textasciicircum\{+0.05\}\$ &  \$-0.89\_\{-0.18\}\textasciicircum\{+0.11\}\$ &  \$0.55\_\{-0.21\}\textasciicircum\{+0.14\}\$ &      6.46 &      6.73 &     -1.25 &       0.342 &       0.306 \\
GRB160118060 &  \$-0.54\_\{-0.16\}\textasciicircum\{+0.13\}\$ &  \$-0.79\_\{-0.19\}\textasciicircum\{+0.15\}\$ &  \$0.22\_\{-0.22\}\textasciicircum\{+0.17\}\$ &      9.30 &      1.41 &     -4.00 &       0.844 &       0.834 \\
GRB160215773 &  \$-0.92\_\{-0.07\}\textasciicircum\{+0.06\}\$ &   \$0.06\_\{-0.69\}\textasciicircum\{+0.57\}\$ &  \$2.96\_\{-1.29\}\textasciicircum\{+1.05\}\$ &     19.55 &      4.46 &     -7.91 &       0.862 &       0.880 \\
GRB160422499 &  \$-0.82\_\{-0.02\}\textasciicircum\{+0.02\}\$ &  \$-0.79\_\{-0.08\}\textasciicircum\{+0.06\}\$ &  \$0.72\_\{-0.16\}\textasciicircum\{+0.14\}\$ &     50.64 &      6.80 &    -17.48 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
GRB160521385 &  \$-0.38\_\{-0.05\}\textasciicircum\{+0.04\}\$ &  \$-0.47\_\{-0.13\}\textasciicircum\{+0.09\}\$ &  \$0.58\_\{-0.12\}\textasciicircum\{+0.12\}\$ &     20.82 &      6.76 &     -4.74 &       0.700 &       0.034 \\
GRB160530667 &  \$-0.54\_\{-0.03\}\textasciicircum\{+0.03\}\$ &  \$-0.69\_\{-0.05\}\textasciicircum\{+0.04\}\$ &  \$0.42\_\{-0.07\}\textasciicircum\{+0.06\}\$ &     17.84 &      6.97 &      6.47 &  \$<10\textasciicircum\{-3\}\$ &  \$<10\textasciicircum\{-3\}\$ \\
\bottomrule
\end{tabular}

